Sampling and Reconstructing Angular Domains with Uniform Arrays

The surge of massive antenna arrays in wireless networks calls for the adoption of analog/hybrid array solutions, where multiple antenna elements are driven by a common radio front end to form a beam along a specific angle in order to maximize the beamforming gain. Many heuristics have been proposed to sample the angular domain by trading off between sampling step size and overhead, where arbitrarily small angular step size is only attainable with infinite sampling overhead. We show that, for uniform linear and rectangular arrays, lossless reconstruction of the array's angular responses at arbitrary angular precision is possible using a finite number of samples without resorting to assumptions of angular sparsity. The proposed method, sampling and reconstructing angular domain (SARA), defines how many and which angles to be sampled and the corresponding reconstruction. This general solution to scan the angular domain can therefore be applied not only to beam acquisition and channel estimation, but also to radio imaging techniques, making it a candidate for future integrated sensing and communications (ISAC). Extensive simulation results for target detection and radio imaging have demonstrated clear advantages of SARA versus other considered baselines, both in terms of angular reconstruction performance and computational complexity.

==> Content/CircularArrays.tex <==
\section{Extension to Circular Arrays - Not this paper}\label{sec:CircularArrays}
\subsection{Circular Transforms}
\subsection{LAD simplification with asin and sin relationship}

==> Content/EquivalentDigital.tex <==
\section{Equivalent Digital Signals - Not this paper}\label{sec:EquivalentDigital}
\subsection{Equivalent Digital Signal from Analog scans}
\subsection{Super Resolution Methods available}

==> Content/MultipleTargets_old.tex <==
\subsection{Reconstruction results - Multiple targets}

\if\single1
\begin{figure*}[ht]
        \centering
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/FA_Rate_NAF_Sweep_16.tikz}
            \caption{$P^\text{(FA)}$, $N=16$.} 
            \label{fig:FA_Rate_NAF_Sweep_16}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/Missed_Det_NAF_Sweep_16.tikz}
		    \vspace{-0.46cm}
		    %\vspace{-0.73cm}
            \caption{$P^\text{(MD)}$, $N=16$.} 
            \label{fig:Missed_Det_NAF_Sweep_16}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/RMSE_NAF_Sweep_16.tikz}
            \caption{\gls{LAD} \gls{RMSE}, $N=16$.}  
            \label{fig:RMSE_NAF_Sweep_16}
        \end{subfigure}
        \vskip\baselineskip
        \vspace{-0.5cm}
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/FA_Rate_NAF_Sweep_128.tikz}
			\vspace{-0.46cm}
            \caption{$P^\text{(FA)}$, $N=128$.} 
            \label{fig:FA_Rate_NAF_Sweep_128}
            \vspace{0.3cm}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/Missed_Det_NAF_Sweep_128.tikz}
            \caption{$P^\text{(MD)}$, $N=128$.} 
            \label{fig:Missed_Det_NAF_Sweep_128}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/RMSE_NAF_Sweep_128.tikz}
            \caption{\gls{LAD} \gls{RMSE}, $N=128$.}  
            \label{fig:RMSE_NAF_Sweep_128}
        \end{subfigure}
        \centerline{\ref{named}}
        \caption{Probability of false alarm, probability of missed detection, and \gls{LAD} \gls{RMSE} of a scenario with three targets and increasing minimum \gls{LAD} spacing between them. All \gls{SARA} curves are with uniform sampling in the \gls{LAD} domain (solid), while for ``CUBIC'' interpolation also uniform sampling of the angles is considered (dashed). All proposals are evaluated at different noise powers $\sigma_n^2=\{-5, -30\}$~dB, marked with circles, and squares, respectively. A default value of $\kappa = 6$ is used, apart from the $P^\text{(FA)}$ figures, where $\kappa=0$ is plotted with dotted curves. The red vertical lines indicate the resolution of the Dirichlet Kernels used for reconstruction.} 
\label{fig:NAF_Sweep}
\end{figure*}
\else
\begin{figure*}[ht]
        \centering
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/FA_Rate_NAF_Sweep_16.tikz}
            \caption{$P^\text{(FA)}$, $N=16$.} 
            \label{fig:FA_Rate_NAF_Sweep_16}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/Missed_Det_NAF_Sweep_16.tikz}
		    \vspace{-0.45cm}
            \caption{$P^\text{(MD)}$, $N=16$.} 
            \label{fig:Missed_Det_NAF_Sweep_16}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/RMSE_NAF_Sweep_16.tikz}
            \caption{\gls{LAD} \gls{RMSE}, $N=16$.}  
            \label{fig:RMSE_NAF_Sweep_16}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/FA_Rate_NAF_Sweep_128.tikz}
			\vspace{-0.45cm}
            \caption{$P^\text{(FA)}$, $N=128$.} 
            \label{fig:FA_Rate_NAF_Sweep_128}
            \vspace{0.2cm}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/Missed_Det_NAF_Sweep_128.tikz}
            \caption{$P^\text{(MD)}$, $N=128$.} 
            \label{fig:Missed_Det_NAF_Sweep_128}
        \end{subfigure}
        \hfil
        \begin{subfigure}[t]{0.325\textwidth}
            \centering
			\input{Figures/RMSE_NAF_Sweep_128.tikz}
            \caption{\gls{LAD} \gls{RMSE}, $N=128$.}  
            \label{fig:RMSE_NAF_Sweep_128}
        \end{subfigure}
        \centerline{\ref{named}}
        \caption{Probability of false alarm, probability of missed detection, and \gls{LAD} \gls{RMSE} of a scenario with three targets and increasing minimum \gls{LAD} spacing between them. All \gls{SARA} curves are with uniform sampling in the \gls{LAD} domain (solid), while for ``CUBIC'' interpolation also uniform sampling of the angles is considered (dashed). All proposals are evaluated at different noise powers $\sigma_n^2=\{-5, -30\}$~dB, marked with circles, and squares, respectively. A default value of $\kappa = 6$ is used, apart from the $P^\text{(FA)}$ figures, where $\kappa=0$ is plotted with dotted curves. The red vertical lines indicate the resolution of the Dirichlet Kernels used for reconstruction.} 
\label{fig:NAF_Sweep}
\end{figure*}
\fi
In this subsection, we consider experiments with $Q=3$ targets placed at random angles, but spaced by at least $\Delta \ell$ in the \gls{LAD} domain. The presence of multiple peaks requires the definition of a peak search routine to detect targets and estimate their angular location and amplitude in the reconstructed response.
We assume that a peak is present if the angular response's magnitude exceeds the \gls{CFAR} threshold given by
\begin{equation}
\zeta = \sqrt{-\sigma^2 \ln(1-(1-P^\text{(FA)})^{\frac{1}{2N -1}})} \; ,
\label{eq:CFAR}
\end{equation}
where $P^\text{(FA)}$ is the desired false alarm probability, defined as the event of detecting a peak where only noise was present~\cite{richards2014principles}.
\if\onappendix1
For the derivation of \eqref{eq:CFAR}, please refer to Appendix \ref{app:CFARDerivation}.
\else
For the derivation of \eqref{eq:CFAR}, please refer to Appendix D of the supplementary material, where we compute $\zeta$ such that the probability of a noise sample's amplitude to exceed it is the desired $P^\text{(FA)}$.
\fi
In our study, we chose $P^\text{(FA)} = 10^{-3}$. Moreover, a detected peak is considered as a false alarm if it is more than $1/(2N-1)$ \gls{LAD} away from a true target, i.e. the Dirichlet kernel's main lobe half width. For the detection of multiple targets using reconstruction techniques (\gls{SARA} and CUBIC), we iteratively scan the reconstructed angular response for the strongest remaining peak. We can then coherently remove the $i$-th iteration's target contribution to get the angular response for the next iteration as
\begin{equation}
R_{i+1}(l) = R_{i}(l) - R_i\left(\hat{\eta}_i \right) \cdot  \left( D_{N} \left( \ell - \hat{\eta}_i \right) \right)^2 \;,
\label{eq:PeakRemoval}
\end{equation}
where $\hat{\eta}_i$ is the \gls{LAD} estimate of the $i$-th iteration's target. Notice the squaring of $D_N(l)$, which is due to the multiplying effects of transmitter and receiver, as introduced in Subsection \ref{subsec:DirectionalTxRx}. After the cancelation of peaks generated by multiple interfering targets, false residual peaks may be created at iterations $i > 1$. We prevent their detection by rejecting peak estimates if there was no peak in the original $R_1(l), l \in [\hat{\eta}_i - 1/(2N-1), \hat{\eta}_i + 1/(2N-1)]$.
Finally, sidelobes and inter-target interference can cause additional detections, especially in low-noise scenarios where $\zeta^{(\text{CFAR})}$ is low. To account for this, the threshold is updated after the first peak's detection as 
\begin{equation}
\zeta' = \max{\Big\{\zeta , \; \kappa \cdot S_{N} \cdot R_1\left(\hat{\eta}_1 \right)\Big\}} \;,
\label{eq:CFARAdaption}
\end{equation}
where $S_N$ is the first sidelobe's relative amplitude of the used Dirichlet Kernel \cite{johnson1992array}, and $\kappa$ a scaling factor chosen based on experiments and tuned such that the desired $P^\text{(FA)}$ can be approximately attained. We found $\kappa = 6$ to be a suitable value in our scenario. For MUSIC, the peak search routine returns the $\hat{Q}$ strongest peaks, where $\hat{Q}$ is estimated with the \gls{MDL} criterion.

\todo[inline]{SM: this text explanation must be reduced. The current version is too long. I tried changing a bit the text and added some suggestions inline, but the more I read this, the more I think that a complete restructure of this subsection is necessary.}
Fig.~\ref{fig:NAF_Sweep} shows the probability of false alarm $P^\text{(FA)}$, probability of missed detection $P^\text{(MD)}$, defined as the percentage of undetected targets, and \gls{LAD} \gls{RMSE} curves with $N=16$ and $N=128$.
% for our considered simulation scenario with $N=8$ (first row) and $N=16$ (second row) antenna elements, respectively. For our analysis, we define $P^\text{(MD)}$ as the percentage of targets that remain undetected. 
For reconstruction techniques, we compare the optimal case of \gls{SARA} with uniform \gls {LAD} sampling (``\gls{SARA} \gls{LAD}'') against cubic interpolation with uniform \gls{LAD} sampling (``CUBIC \gls{LAD}''), and the worst baseline with cubic interpolation and uniform sampling in the angular domain (``CUBIC Angle''). As super resolution baseline, we investigate MUSIC's performance both with uniform \gls{LAD} sampling (``MUSIC \gls{LAD}'') and uniform sampling in the angular domain (``MUSIC Angle''). Each curve is evaluated at noise powers $\sigma_n^2$ of $-5$~dB and $-30$~dB. \revi{rev:resolution}{The vertical curves representing the Rayleigh criterion for resolution of two targets~\cite{johnson1992array} are also added, corresponding to the Dirichlet kernel's main lobe half width.}

\todo[inline]{SM: maybe I am forgetting something, but with MUSIC there is no way to keep FA under control, but this depends on the MDL behavior, right? Shall we mention this? Moreover, I'd make more clear the fact that $\kappa = 6$ is used only with SARA and CUBIC. In order to reduce curves and save space,  we can maybe remove the $\kappa = 0$... Any other suggestion?}
Observing the $P^\text{(FA)}$ curves in the first column of Fig. \ref{fig:NAF_Sweep}, it can be seen that for $\sigma_n^2 = -5$~dB and $N=16$ the desired $P^\text{(FA)}$ is almost achieved for ``\gls{SARA} \gls{LAD}'' and ``CUBIC \gls{LAD}''. The slight mismatch is due to an imperfect target estimation and removal in this high noise scenario, where
%$\zeta$~\eqref{eq:CFARAdaption} defaults to $\zeta^{(\text{CFAR})}$~\eqref{eq:CFAR}
 $\zeta$~\eqref{eq:CFAR} is by itself high enough not to require any enhancements, i.e., $\zeta'=\zeta$. In other scenarios, however, interference and sidelobes exceed the initial \gls{CFAR} threshold, such that $\zeta'$ is raised after the first detection. The curves with $\kappa = 6$ show that in low-noise regimes false alarms can always be avoided once targets are fully resolvable and do not interfere with each other anymore. %The authors want to highlight that the choice of $\kappa = 6$ does not impact $P^\text{(MD)}$ in our experiments, but only reduces $P^\text{(FA)}$.
 Finally, to justify the need for (\ref{eq:CFARAdaption}), we also plot the curves with $\kappa = 0$, that exhibit an uncontrollable $P^\text{(FA)}$.
 \todo[inline]{We may remove the next sentence, but it may expose the work to a non-careful reviewer's attacks, what do you think?}
 Note that values above one can occur, as per our definition $P^\text{(FA)}$ describes the expected number of false alarms per experiment. At both noise powers, MUSIC exhibits higher false alarm rates compared to the reconstruction techniques \gls{SARA} and CUBIC. 
The $P^\text{(MD)}$ curves in Figs.~\ref{fig:Missed_Det_NAF_Sweep_16} and \ref{fig:Missed_Det_NAF_Sweep_128} show that \gls{SARA} yields minor, but consistent, resolution gains compared to ``CUBIC \gls{LAD}'', enhancing the ability to resolve multiple targets.
\todo[inline]{MH: the following sentence is still to be modified based on the final results with 1e6 experiments} As an example, to achieve a $P^\text{(MD)}$ of $10^{-4}$ with $N=16$, \gls{SARA} needs roughly 8\% less \gls{LAD} spacing at $\sigma_n^2 = -30$~dB than the ``CUBIC \gls{LAD}'' baseline. The resolution gains slightly diminish, but are still significant for $N=128$. Note that for uniform \gls{LAD} sampling, $P^\text{(MD)}$ starts to drop after $\Delta \ell$ reaches the Dirichlet Kernel's main lobe half width of $1/(2N{-}1)$ in \gls{LAD}. Nonetheless, the "waterfall" does not happen immediately after this point due the presence of sidelobes making the targets interfere with each other even after this resolution value. When sampling the angular domain uniformly, however, the targets become resolvable only considerably later. As expected, due to its super-resolution properties, MUSIC improves the capability to discriminate close targets in low-noise regimes compared to the reconstruction techniques. However, it can clearly be seen that uniform \gls{LAD} sampling is pivotal also for MUSIC, as ``MUSIC Angle'' performs drastically worse and is not able to resolve the three targets reliably.
%This further stresses the importance of sampling in the \gls{LAD} domain.

The corresponding \gls{LAD} \gls{RMSE} curves of Figs.~\ref{fig:RMSE_NAF_Sweep_16} and \ref{fig:RMSE_NAF_Sweep_128} account for missed detections with an error of $\sqrt{3}/4$ in \gls{LAD}, corresponding to the maximum possible angle $\theta^\text{max} = \pi/3$ rad. % 
The curves show similar patterns compared to the previously analyzed results and validate \gls{SARA}'s benefits over ``CUBIC'' for multi-target scenarios. Moreover, if the targets are fully resolvable, \gls{SARA} is also able to outperform MUSIC in terms of \gls{LAD} \gls{RMSE}.

In summary, the results confirm that \gls{SARA} is the superior reconstruction technique compared to the ``CUBIC'' baselines also in multi-target scenarios, even if the optimal angular sampling criterion - \gls{LAD} - is applied also for ``CUBIC''. Furthermore, \gls{SARA} achieves a lower \gls{LAD} \gls{RMSE} floor than MUSIC, while losing in target detection capability due to MUSIC's super-resolution capabilities.

%In summary, the results with multiple targets confirm that \gls{SARA} can reduce the \gls{LAD} \gls{RMSE} compared to the ``CUBIC'' baselines. Moreover, \gls{SARA} offers an increased capability to resolve targets, even if the optimal angular sampling criterion - \gls{LAD} - is applied also for ``CUBIC''.

%., while at the same time achieving a significantly lower false alarm rate in low-noise scenarios.

%To account for targets' sidelobes, that may interfere with each other and can exceed the \gls{CFAR} threshold, we additionally require each peak to have a \gls{TP} of $P = \frac{1}{4}N$. This value is chosen based on experiments and tuned such that the desired false alarm probability can be attained.


%\textcolor{red}{Note that, while this value can be achieved when there is only noise (no target), it is merely an approximation in the presence of scatterers due to the sidelobes arising from the Dirichlet Kernel, which can be higher than the originally defined threshold. To account for this, we iteratively scan the reconstructed angular response for the strongest remaining peak and after each detection raise $\zeta$ by the estimated magnitude of the first sidelobe. We thereby make sure that $P_{FA}$ is never exceeded in our simulations. A more elaborate \gls{CFAR} adaptive threshold computation is out of the scope of this work and subject of future work.}

%Interestingly, for both $N=8$ and $N=16$ with \gls{LAD} sampling, \gls{SARA} is able to achieve almost the same performance with $\sigma_n^2 = -10$~dB as the ``CUBIC \gls{LAD}'' baseline with $\sigma_n^2 = -30$~dB, both in terms of \gls{LAD} \gls{RMSE} and $P^\text{(MD)}$.

%\todo[inline]{I'm not super happy with $S_N$, do you think it's okay? Maybe we can even define the strongest sidelobes's amplitude in terms of $D_N(x)$, with x being the angular location of the strongest sidelobe, assuming a target at 0 NAF (I guess it can be expressed in terms of the resolution somehow)? What do you think?}

%Lastly, Fig. \ref{fig:FA_Rate} demonstrates that with our peak detection routine and \gls{SARA} we are able to attain the desired $P^{\text{(FA)}}$. Note that in the high-noise scenario ($\sigma_n^2=-5$~dB), $\zeta$ defaults to the theoretical \gls{CFAR} threshold, as it is much higher than the sidelobe level. Hence, $P^{\text{(FA)}}$ is reasonably achieved for both ``\gls{SARA} \gls{LAD}'' and ``CUBIC \gls{LAD}''. At $\sigma_n^2=-30$~dB however, the sidelobes exceed the initial \gls{CFAR} threshold such that it is raised after the first detection according to (\ref{eq:CFARAdaption}). For \gls{SARA}, this adaptation achieves a false alarm rate of roughly $10^{-5}$ for $N=8$ and prevents false alarms for $N=16$. On the other hand, with cubic interpolation, $P^{(FA)}$ is above the desired level due to reconstruction errors exceeding even the raised threshold.

%Furthermore, starting with the second detection, we additionally scan the original reconstructed angular response $R_1(l)$ around the peak locations to prevent the detection of artificially created artifacts. Those can arise if the detection is due to interference of unresolvable targets, causing wider peaks that do not match the shape of the Dirichlet Kernel that is used for coherent removal. 

%\todo[inline]{SM: I would explain everything without $k$, rephrasing the previous paragraph into something simpler, like, ``On top of coherent removal as in \eqref{eq:PeakRemoval}, we reject peaks that were not present in the initial $R_1(l)$.'' (btw, how can you do it precisely?) ``After cancellation of peaks generated by multiple interfering targets, false residual peaks may be created and we want not to detect them''. 

%Then, I would start explaining $P_FA$, why it does not work without $k$, and then you introduce \eqref{eq:CFARAdaption}

%Please, rephrase a bit what follows accordingly, shrinking a bit the text (if you can, otherwise I take care of it) and going to the point.}


==> Content/RevisionAnswers_firstReview.tex <==

\clearpage

\section*{Answer to the Editor and Reviewers' Comments}

The authors thank the Editor and the Reviewers for their comments and support which help to improve the paper. 
%
We have carefully addressed each of the comments raised and provided a point-by-point response below.   Substantial text changes  are highlighted as \underline{underlined texts}
 in the main body and are subsequently quoted in our responses below.  

\section*{Editor}
 

~\\ \noindent{\bf (1) The reviewers have raised some concerns about this work. The novelty and contribution in this work need to be clearly discussed in more detail, in light of existing works as pointed out by the reviewers. Multiple reviewers raised concerns about the current introduction in Section I, where the problem is not well-motivated, the discussion needs to be refocused on the related work surrounding the problem considered, and the contribution of this work needs to be more detailed with the novelty better highlighted. Also, more simulation results with a broader value of system parameters should be provided. The overall writing should be carefully revised for improvement. The reference style should be carefully checked, and discrepancies in single- and double-column versions should be removed. 
%Based on the review comments, your manuscript is received major revision decision. Please carefully revise the manuscript to address reviewer comments and concerns and provide point-to-point response.
 }
\setstretch{1.5} 

~\\ \noindent{\bf Ans:} Thanks for your comment. We tried to address all of your concerns, improving the paper through the following big areas
\begin{itemize}
    \item Section \ref{sec:Intro} has been reshaped to offer a better context for the problem addressed in this work, highlighting more prior art and better addressing our contribution.
    \item The mathematical derivations have been simplified to improve readability without implications on the final results.
    \item Simulation experiments have been extended, following the reviewers' suggestions and two super-resolution baselines have been added.
    \item We reviewed the computational complexity part, improving it based on the comments of reviewer 2.
    \item An overall writing and reference style review has been done.
    \item An error in the derivation  for the \gls{URA} extension in Subsection \ref{subsec:URAExtension} has been spotted and corrected.
\end{itemize}

Moreover, the authors would like to give a further explanation on the detection threshold adaption \eqref{eq:CFARAdaption}, which due to space reasons had to be omitted from the paper, but helps to further clarify its necessity. Fig. \ref{fig:Kappa_0_P_FA_Example} clearly shows that choosing $\kappa=0$ leads to uncontrollable false alarm rates for both ``\gls{SARA} \gls{LAD}'' (blue) and ``CUBIC \gls{LAD}'' (green). This is due to the fact that in low noise scenarios interference and sidelobes of the Dirichlet Kernel used for reconstruction can cause artificial peaks that easily exceed the theoretical \gls{CFAR} threshold $\zeta$~\eqref{eq:CFAR}, requiring further measures to keep $P^\text{(FA)}$ under control. Note that values above one can occur, as per our definition $P^\text{(FA)}$ describes the expected number of false alarms per experiment. The solid curves show that by choosing $\kappa=6$ the desired $P^\text{(FA)}$ of $10^{-3}$ can approximately be attained. Furthermore, false alarms can be completely avoided once targets become fully resolvable. In high noise scenarios ($\sigma_n^2 = -5$~dB), $\zeta$~\eqref{eq:CFAR} is by itself high enough to not require any enhancements, i.e. $\zeta'=\zeta$.

\begin{figure}[t!]
  \centering
  \input{Figures/FA_Rate_NAF_Sweep_16_kappa_0.tikz}
  \caption{Probability of false alarm of a scenario with three targets and increasing minimum \gls{LAD} spacing between them at noise power $\sigma_n^2=-30$~dB and with $N=16$ antennas. Our proposal ``\gls{SARA} \gls{LAD}'' (blue) is compared to ``CUBIC \gls{LAD}'' (green). Solid lines represent $\kappa = 6$, while the dotted lines correspond to $\kappa = 0$, i.e no peak threshold adaption.}  % subcaption
\label{fig:Kappa_0_P_FA_Example}
\end{figure}


\newpage
\section*{Reviewer: 1}

~

\setstretch{1.0}

\noindent {\bf In this manuscript, the authors propose a new method for array angular response reconstruction using finite samples that do not exploit the assumption of sparsity properties.
The reviewer thinks the manuscript can be improved if the authors consider the problems:}
\setstretch{1.0}


~\\ \noindent{\bf 1) The introductory part of the manuscript should be embellished. For example, the hybrid array can be briefly summarized and the author should focus on the motivation of the research content to make it more logical.}
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We agree with the reviewer that some restructuring of the introduction is needed. We took some actions in this direction, hoping to have solved this issue that all the reviewers pointed us to. In particular, we tried highlighting the importance of network sensing in future \gls{6G} standards, in addition to the well-known channel estimation problem. Then, the following text tries to recap why our contribution is relevant at the light of the two problems recalled above.

``\revp{rev:ImagingIntro}  However, we show in our numerical evaluations that the proposed non-sparse reconstruction is valid also to estimate the sparse angular components of wireless channels, that is the typical assumption for \gls{mmWave} and higher carrier frequency systems~\cite{alkhateeb2013hybrid}.''

%\hl{Rev is bugged here, therefore changes to text should be reflected to this.}

\setstretch{1.5}

~\\ \noindent{\bf 2) The author should recheck some details of the article, such as the explanation of abbreviations using repetitive issues like SARA, which has been explained in the previous article and re-explained again in the later article.}
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the comment. We have carefully revised the manuscript and removed repetitive definitions. 

%We are not sure about the ``previous article'' reference by the reviewer. We want to stress that this publication contains material never published by the authors. An ArXiv preprint has been released after the first TWC submission, in agreement with the editor. However, we agree that some of the wording in this article can be improved and we tried working at it. 

%\hl{Does this answer make sense? To be honest, I am not sure of what the reviewer meant}
\setstretch{1.5}

~\\ \noindent{\bf 3) The parameter settings of the experimental part should be applicable to the massive MIMO scenario, the authors use a maximum of 64 antennas to verify the proposed method, we recommend that the experimental verification be performed at 128 antennas or more.}
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the comment.
We want to remark that the angular resolution of a $N=64$ \gls{ULA} would be the same as a $64$x$64$ \gls{URA} that has $4096$ elements uniformly spaced in the \gls{2D} panel. This is why we did not consider higher number of antennas for \glspl{ULA}.

Taking the reviewer's comment into account, we anyway modified our Figs.~\ref{fig:RMSE_Variable_Antennas} and \ref{fig:RMSE_Peak}  to include $N=128$ results,  dropping $N=64$ to avoid crowded plots. 
The same was done in Fig.~\ref{fig:NAF_Sweep}.

\setstretch{1.5}

~\\ \noindent{\bf 4) The authors point out in the abstract that the proposed method can be applied to channel estimation, and what are the steps for applying this method to channel estimation.}
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for pointing out this lack of information. We added the following text in the introduction Section

``\revp{rev:ChannelEstimationIntro}'' 

and the following text in the numerical experiments Section

``\revp{rev:ChannelEstimationSimulation}'' 

%\hl{Jinfeng, please have a crack at it once our intro review has been completed. Maybe we want to add something different (even somewhere else)}

%\hl{Add that with IDFT tricks one can get the signal at each antenna element}
\setstretch{1.5}

~\\ \noindent{\bf 5) For the reference section, please follow the standard journal article citation format and increase the number of articles cited.}
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the suggestion. We hope to have correctly harmonized the references Section's formatting, taking as example other published TWC papers. Some references (like the ones suggested below) have been added based on other comments and the new material in this manuscript revision.
\setstretch{1.5}

~\\ \noindent{\bf 6) Some of the latest works  are missed, e.g., "Joint Estimation of Multipath Angles and Delays for Millimeter-Wave Cylindrical Arrays With Hybrid Front-Ends," in IEEE Transactions on Wireless Communications, vol. 20, no. 7, pp. 4631-4645, July 2021. "Nested Hybrid Cylindrical Array Design and DoA Estimation for Massive IoT Networks," in IEEE Journal on Selected Areas in Communications, vol. 39, no. 4, pp. 919-933, April 2021. }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} Thanks for pointing us to these references.
Reference 1, now cited as~\cite{lin2021joint}, focuses on signal model
and angular sampling of \glspl{UCyA} and proposes a linear angular interpolation between angular samples. Reference 2, now cited as~\cite{lin2020nested}, adopts sparse array techniques for nested hybrid \glspl{UCyA}. However, as acknowledged in~\cite{lin2021joint} and demonstrated in this work, linear angular interpolation is not the correct approach for \glspl{ULA} and \glspl{URA}. In particular, the Whittaker-Shannon interpolation  would require infinite contributions and would be therefore noisy in practice (see our equation~\eqref{eq:InfiniteReconstructionSummation}). In contrast, in this work we show how lossless reconstruction can be obtained without infinite summation of contributions (see for instance~\eqref{eq:InterpolationGenericFinal}), solving the issue mentioned by the references.
Since both approaches are dealing with \glspl{UCyA}, they are not tailored for the signal model and issues generated by \gls{ULA} and \gls{URA}. Therefore, we did not implement these algorithms as baselines. 

In summary,  the two references propose interesting hybrid beamforming techniques with \glspl{UCyA} and associated angular sampling and interpolation methods. We acknowledge that the references should be part of the prior art and are cited with the following added text in the introduction.

\setstretch{1.5}

"\revp{rev:newRef}"

%\hl{Jinfeng, please review this}
%\hl{We need to address Reviewer 3's comment "The overall algorithm designed in this paper comprises a series of conventional ideas" as well here by explicitly emphasizing the creative steps in SARA that are specialized to the necessary and sufficient amount of sampling and lossless reconstruction.}

\newpage
\section*{Reviewer: 2}

~

\setstretch{1.0}

\noindent {\bf The work presented is mathematically sound and well-presented. Extensive simulation results are presented to benchmark the proposed algorithm in different environments.  Some minor comments are provided here to clarify some aspects. }
\setstretch{1.0}


~\\ \noindent{\bf 1) Typo: when referring to the figures, the same format as the caption should be used in the text, e.g. Fig. x. }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the correction. We hope to have corrected it properly.
\setstretch{1.5}

~\\ \noindent{\bf 2) Current ref[10] (new~\cite{zhang2021gridless}) also investigates the fact that, in the transformed domain, the signal can be seen as a sum of sinusoids, and the frequency estimation arises (see follow-up paper https://ieeexplore.ieee.org/abstract/document/9569292 - Low-complexity AoA and AoD Estimation in the Transformed Spatial Domain for Millimeter Wave MIMO Channels). It might be interesting to compare both algorithms to some extend, although TSDCE is applied to sparse channels. }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the suggestion. We implemented the \gls{TSDCE} algorithm, with a slight modification from the  original work in~\cite{zhang2021gridless}, where the number of targets is assumed to be known. In our work, we applied the \gls{MDL} criterion~\cite{rissanen1978modeling} to determine the model order, as we did for the MUSIC baseline.

%\hl{Not sure if we want to put the sentence above in the main text}
%\textcolor{red}{MH: I would not. Actually to me it's not even entirely clear why it is here.}
Accordingly, TSDCE curves are added in the single target \gls{LAD} estimation curves (Fig. \ref{fig:RMSE_Variable_Antennas}), along with the following text:

"\revp{rev:TSDCE_Results}"

To expand on the previous explanation given in the paper, the additional provided Fig.  \ref{fig:RMSE_Variable_Antennas_Translated} plots the same curves as Fig. \ref{fig:RMSE_Variable_Antennas}, where \gls{TSDCE} noise has not been enhanced by the $\frac{N^2}{2N-1}$ factor described in Section~\ref{sec:Simulation}. One can immediately notice that for both $N = \{16, 128\}$ \gls{TSDCE} would outperform the \gls{CRLB}. 

On the other hand, applying the noise scaling according to the additionally necessary scans to have a fair comparison, as in Fig.~\ref{fig:RMSE_Variable_Antennas}, causes \gls{TSDCE} to exhibit a worse performance than the other baselines. However, the authors want to explicitly emphasize that this does not reduce \gls{TSDCE}'s contributions. In fact, \gls{TSDCE} is designed to work on the two-dimensional problem of estimating angles of arrival/departure, while our scenario is tailored to a single dimension use case. For the considered mono-static radar scenario, this requires acquiring many ``useless" scans to apply \gls{TSDCE}, focusing also on angle of departures that are considerably different than angle of arrival, where no target has a meaningful contribution. Therefore, the number of ``interesting" samples is only a small subset of $N^2$. 
%One countermeasure could be to estimate the cardinality of this subset of interesting samples and scale the noise accordingly. However, this clearly has the drawback of integrating a heuristic into the comparison, which is why we decided against it. 
We hope this suffices to explain why i) noise scaling for \gls{TSDCE} is necessary in order to comply with theoretical bounds, and ii) a fair comparison with \gls{TSDCE} is not trivial, which is why it is dropped from our analysis after Fig.~\ref{fig:RMSE_Variable_Antennas}.

%\hl{JD: the conference version, referred by the reviewer, is not included in the reference list yet. Since \gls{TSDCE} is designed for communication (bi-static sensing), we have to set $n_T=n_R=N$ and do $N^2$ samples to make \gls{TSDCE} suitable for mono-static sensing setup that paper is addressing. Could we use this as an argument to further justify why a direct comparison is non-trivial and re-scaleing SNR is not perfect but reasonable? Alternatively, I have no problem in saying that \gls{TSDCE} performs better or even exceed CRA because it uses two radios (bi-static) and $N/2$ times more sampling. 
%MH: I agree with Jinfeng that the conference version should also be referenced in our paper. Should we replace the journal version with it or reference both?

%SM: let's keep both of them. Marcus, please resolve this and delete our comments.}

\begin{figure}
  \centering
%  \includegraphics[width=1.0\columnwidth]{Figures/RMSE_Variable_Antennas.png}
  \input{Figures/RMSE_Variable_Antennas_translated}
  \caption{\gls{RMSE} of single target \gls{LAD} estimation using \glspl{ULA} with variable number of 
  %$N=16$ (dashed lines) and $N=128$ (dotted lines) \
  antennas. 
  %The \glsentrylong{CRLB} (\glsentryshort{CRLB}) of equation \eqref{eq:CRLB} is plotted with cyan curves.} % subcaption
  }
  \label{fig:RMSE_Variable_Antennas_Translated}
\end{figure}
\setstretch{1.5}

~\\ \noindent{\bf 3) In the simulations section, although the authors indicate the reason not to include algorithms featured for sparse channels, it might be interesting to add them as a benchmark.  }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the suggestion. As a further benchmark, we added the well-known MUSIC algorithm as a super-resolution technique that can be used to estimate sparse components. Moreover, we also investigated \gls{TSDCE}'s application to our problem (see previous comment).
\setstretch{1.5}

~\\ \noindent{\bf 4) Regarding the discussion about complexity (page 7, line 44), the execution time might not be the best metric and the trend might not hold for different platforms. As future work, the authors should consider analyzing efficient implementation of their algorithm, for example using multi-core or gpu architectures. The current paragraph regarding the execution time should be revised.}
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the suggestion. The final solution we propose (\gls{AR}) is dominated by the complexity of the IDFT and DFT operations, that are already optimized by most common numeric computation libraries, like NumPy, C++ and even FPGAs. We therefore rely on this existing work and use NumPy libraries to execute our code.

We agree with the reviewer that execution time is not a reliable metric to evaluate complexity. Even though in the initial submission we put the corresponding figure to showcase that also with a small number of $N$ one can practically observe consistent complexity gains, we decided to remove it based on this comment, leaving only a table, summarizing the order of complexity for every considered algorithm. We have therefore modified the text on complexity as follows

``\revp{rev:complexity}''
\setstretch{1.5}

\newpage
\section*{Reviewer: 3}

~

\setstretch{1.0}

\noindent {\bf In this manuscript, the authors provided the theory to sample and reconstruct the angular response of ULA and practical applications of the theory to sensing use cases. The reviewer has the following concerns, especially about the alignment with TWC and the novelty/clarity.  }
\setstretch{1.0}


~\\ \noindent{\bf 1) First, the number of references differs between the single-column and double-column versions. Second, the review can’t find the reference called “[20] S. Mandelli, M. Henninger, and J. Du, ‘Sampling and reconstructing angular domains with uniform arrays,’ 2022” cited in the body of the double-column version. Moreover, the format of the references section needs to be checked.  }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} Thanks for this observation. We harmonized references and their style. In the final version of the paper, if there is not enough space for all the additional derivations in the appendixes and the editor is ok with it, we plan on transferring some of the derivations to an online version of the paper and properly reference it. 

\setstretch{1.5}

~\\ \noindent{\bf 2) The reviewer suggests reorganizing the introduction. In particular, the first two paragraphs are not closely related to this manuscript. Additionally, the related work is less described, and the motivation is unclear. This actually leads to my concern if the paper is best aligned with the scope of TWC, or maybe TAP or TSP could be the better venue for the paper.  }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:}
We thank the reviewer for the suggestion. We reviewed the introduction according to your feedback. Regarding the paper's scope: we believe that TWC is a better fit, due to the need of angular sampling imposed by analog (and hybrid) arrays, that are currently the most used solutions for carrier frequencies above 6 GHz. In particular, this work is of particular relevance with the surge of the network sensing use cases for future \gls{6G} networks, where imaging with analog/hybrid arrays will become as relevant as sparse channel estimation techniques. We tried to improve the context accordingly in the introduction Section. In particular, we tried improving the clarity of the problem definition with the following text.

``\revp{rev:ProblemSummary}''
\setstretch{1.5}

~\\ \noindent{\bf 3) The overall algorithm designed in this paper comprises a series of conventional ideas. The authors are expected to articulate the novelty of problem formulation, methodology, and finding. The current structure of Sec. I-A is hard to follow and subsequently lacks clarity of the novelty compared with some recent relevant works, e.g.,
\begin{itemize}
    \item [R1] “Joint Estimation of Multipath Angles and Delays for Millimeter-Wave Cylindrical Arrays with Hybrid Front-Ends," IEEE Trans. Wirel. Comm., vol. 20, no. 7, pp. 4631 – 4645, July 2021.
    \item [R2] “Nested Hybrid Cylindrical Array Design and DoA Estimation for Massive IoT Networks,” IEEE J. Select. Areas Comm., vol. 39, no. 4, pp. 919 – 933, April 2021. 
\end{itemize}

  }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for pointing us to these references, which have also been suggested by reviewer 1. Below we comment on the cited references, and we tried improving clarity across the paper to motivate our work. 

Reference R1, now cited as~\cite{lin2021joint}, focuses on signal model
and angular sampling of \glspl{UCyA} and proposes a linear angular interpolation between angular samples. Reference R2, now cited as~\cite{lin2020nested}, adopts sparse array techniques for nested hybrid \glspl{UCyA}. However, as acknowledged in~\cite{lin2021joint} and demonstrated in this work, linear angular interpolation is not the correct approach for \glspl{ULA} and \glspl{URA}. In particular, the Whittaker-Shannon interpolation  would require infinite contributions and would be therefore noisy in practice (see our equation~\eqref{eq:InfiniteReconstructionSummation}). In contrast, in this work we show how lossless reconstruction can be obtained without infinite summation of contributions (see for instance~\eqref{eq:InterpolationGenericFinal}), solving the issue mentioned by the references.
Since both approaches are dealing with \glspl{UCyA}, they are not tailored for the signal model and issues generated by \gls{ULA} and \gls{URA}. Therefore, we did not implement these algorithms as baselines. %, but they will be considered when we will extend the present work to cylindrical arrays. 
%\hl{SM: Are there any other differences? Marcus, please check

%MH: Apart from using UCyAs in both papers and linear interpolation in \cite{lin2021joint}, I don't think there's another difference we can point out. In \cite{lin2020nested}, they are using sparse array techniques applied to UCyAs and design a 2D DoA estimation algorithm for this specific array design. In my opinion, this approach is so far away from what we are doing that it's hard to point out a specific thing that we're doing differently.} 

In summary,  the two references propose interesting hybrid beamforming techniques with \glspl{UCyA} and associated angular sampling and interpolation methods. We acknowledge that the references should be part of the prior art and are cited with the following added text in the introduction.

\setstretch{1.5}

"\revp{rev:newRef}"
%\hl{I think it is better to itermize the key contributions.}

%\hl{Jinfeng to revise this part} \textcolor{red}{Jinfeng: Done.}


\setstretch{1.5}

~\\ \noindent{\bf 4) On page 3, line 47, please explain how to get the value of $B_N$ from Eqn (1). }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the comment. Given the mathematical restyling of this revision, the quantity was not necessary anymore. However, we tried to properly define every other quantity used in the paper.
\setstretch{1.5}

~\\ \noindent{\bf 5) The reviewer wants to know if there is an explicit expression for the upper bound of the resolution of the proposed method.  }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} Thanks for the question. After some careful reasoning, we came to the following conclusion. Regarding the single target \gls{LAD} estimation results, the proposed \gls{CRLB} approximation is still the best option we found for the lower bound of the \gls{LAD} \gls{RMSE}~\eqref{eq:CRLB}. Unfortunately, like many other maximum likelihood estimators in the literature, we did not find a good way to determine an upper bound that can be tight enough.

Regarding multiple target detection and the corresponding resolution, the vertical lines we drew in Fig.~\ref{fig:NAF_Sweep} correspond to the Rayleigh criterion for resolution~\cite{johnson1992array} (not really a true ``formal'' bound) that one could obtain with an antenna sum co-array with \gls{AAL} aperture $(2N-1)\frac{\lambda}{2}/d = 2N-1$.
From~\cite{johnson1992array}:

``\textit{The Rayleigh criterion for resolution states that two waves are resolved if the peak of the aperture smoothing function due to one falls on the first zero of the aperture smoothing function due to the other}''.

In our case, that corresponds to the Dirichlet kernel's main lobe half width $1/(2N-1)$. As one can notice from the results in Fig. \ref{fig:NAF_Sweep}, this criterion offers only an approximation value for the resolution, that in this case is worse.  We therefore added some text in the paper to better characterize the proposed bound.

``\revp{rev:resolution1}''

and

``\revp{rev:resolution2}''

We are not aware of further bounds or conceptually different approximations regarding multiple target angular resolution. In particular, in some works (for example Braun, Klaus Martin. ``OFDM radar algorithms in mobile communication networks,'' \textit{Diss. Karlsruhe, Karlsruher Institut für Technologie (KIT)}, 2014.) the author considers half the value we considered as nominal resolution for time of arrival estimation with radar. However, practical considerations and the results of Fig.~\ref{fig:NAF_Sweep} show that that bound is too optimistic, therefore we did not consider it.

\setstretch{1.5}

~\\ \noindent{\bf 6)  The comparison scheme “CUBIC” is poorly described. Please briefly describe it or provide a relevant reference.  }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} Thanks for pointing out this issue. We modified the text and added a reference in the paper's text, see below 

``\revp{rev:CUBIC}''
\setstretch{1.5}

~\\ \noindent{\bf 7)  The overall writing of the paper could be substantially improved. }
\setstretch{1.5}

~\\ \noindent{\bf  Ans:} We thank the reviewer for the suggestion. We did our best to improve the readability of the document.
\setstretch{1.5}

==> Figures/DirichletExample.tikz.tex <==
\tikzset{mark size=2.5}    
    \begin{tikzpicture}
	\begin{axis}[
    		height = 7cm,
    		xlabel={\gls{LAD} $\ell$},
    		ylabel={$D_N \left( \frac{2d}{\lambda} (\ell - \eta) \right)$},
%    		ymin=0,
%		ymax=18,
		xmin=-0.5,
		xmax=0.5,
		minor tick num=1,
		yminorticks = true,
		enlargelimits = false,
		legend pos=south east,
		grid = both,
    		grid style={solid, black!15},
    		legend columns = 1,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    		legend style={font=\scriptsize},
			legend cell align={left},
		xtick = {-0.5, -0.25, 0, 0.25, 0.5},
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
        tick label style={/pgf/number format/fixed},
		every axis plot/.append style={thick}
		]
		
		\addplot[color=blue] plot table[x index=0, y index=1] {Data/ExportedDirichletExample.txt};
		\addplot[color=green] plot table[x index=0, y index=2] {Data/ExportedDirichletExample.txt};
		\addplot[color=orange] plot table[x index=0, y index=3] {Data/ExportedDirichletExample.txt};
		
%	\legend{$\eta = 0, d = \lambda/2, N = 8$, $\eta = -0.2, d = \lambda/2, N = 15$, $\eta = 0.4, d = 0.7\lambda, N = 8$}
    \legend{{$\eta = 0, d = \lambda /2, N = 8$}, {$\eta = -0.2, d = \lambda/2, N = 15$}, {$\eta = 0.4, d = 0.7\lambda, N = 8$}}
   	
   	\end{axis} 
   	


\end{tikzpicture}


	

		
%	    \addplot +[mark=none, dotted, forget plot, color=red, thick] coordinates {(0.1, 0) (0.1, 1)};		
%		
%    	\addplot[
%   		color=orange,
%   		mark=diamond,
%   		mark repeat = 30,
%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/TROLL_noCCT};
%    	
%	\addplot[
%   		color=green!70!black,
%   		mark=x,
%   		mark repeat = 30,
%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/TROLL_Detach_noCCT};    	
%
%	\addplot[
%   		color=blue,
%   		mark=o,
%   		mark repeat = 30,
%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/TROLL_DetachPeriod};
%    	
%    	\addplot[
%   		color=black,
%%   		mark=triangle,
%%   		mark repeat = 30,
%%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/OLLA_0.03};
%    	
%    	\addplot[
%    		color=black,
%%    		mark=triangle,
%%   		    mark repeat = 30,
%		densely dashdotted,
%%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/OLLA_0.1};
%    	
%    	\addplot[
%    		color=black,
%%    		mark=triangle,
%%   		    mark repeat = 30,
%    		loosely dashed,
%%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/OLLA_0.3};
%	\legend{\gls{TROLL}, \gls{TROLL} \gls{GD},  \gls{TROLL} \gls{GD}+ \gls{CCT}, OLLA 0.03, OLLA 0.1, OLLA 0.3}

==> Figures/RMSE_Variable_Speed_MaxAngle80.tikz.tex <==
\tikzset{mark size=2.5}    
    \begin{tikzpicture}
	\begin{semilogyaxis}[
    		height = 7cm,
    		xlabel={Noise Power $\sigma_n^2$ [dB]},
    		ylabel={\gls{LAD} \gls{RMSE}},
    	ymin=1e-4,
		ymax=3e-1,
		x dir=reverse,
%		xmin=-0.5,
%		xmax=0.5,
		minor tick num=1,
		yminorticks = true,
		enlargelimits = false,
		legend pos=north east,
		grid = both,
    		grid style={solid, black!15},
    		legend columns = 1,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    		legend style={font=\scriptsize},
%		xtick = {-0.5, -0.25, 0, 0.25, 0.5},
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
        tick label style={/pgf/number format/fixed},
		legend cell align={left},
		every axis plot/.append style={very thick}
		]

\def\maxangle{"80.0"}
\def\speed{"0.0"}
	
		\addplot[color=blue, solid, forget plot] plot table[x index=0, y index=1] {Data/NAF_RMSE_SPEED_SPEED_\speed_MANGLE_\maxangle.txt};
		\addplot[color=green, solid, forget plot] plot table[x index=0, y index=2] {Data/NAF_RMSE_SPEED_SPEED_\speed_MANGLE_\maxangle.txt};
			
\def\speed{"50.0"}
	
		\addplot[color=blue, dashed, forget plot] plot table[x index=0, y index=1] {Data/NAF_RMSE_SPEED_SPEED_\speed_MANGLE_\maxangle.txt};
		\addplot[color=green, dashed, forget plot] plot table[x index=0, y index=2] {Data/NAF_RMSE_SPEED_SPEED_\speed_MANGLE_\maxangle.txt};
		
\def\speed{"200.0"}
	
		\addplot[color=blue, dotted, forget plot] plot table[x index=0, y index=1] {Data/NAF_RMSE_SPEED_SPEED_\speed_MANGLE_\maxangle.txt};
		\addplot[color=green, dotted, forget plot] plot table[x index=0, y index=2] {Data/NAF_RMSE_SPEED_SPEED_\speed_MANGLE_\maxangle.txt};

		\addplot[color=blue, solid, draw=none] coordinates {(0, 0.1)};
		\addplot[color=green, solid, draw=none] coordinates {(0, 0.1)};
		\addplot[color=black, solid, draw=none] coordinates {(0, 0.1)};
		\addplot[color=black, dashed, draw=none] coordinates {(0, 0.1)};
		\addplot[color=black, dotted, draw=none] coordinates {(0, 0.1)};
		
	\legend{\gls{SARA}, CUBIC, $\nu=0$ m/s, $\nu=50$ m/s, $\nu=200$ m/s}
   	
   	\end{semilogyaxis} 

\end{tikzpicture}


	

		
%	    \addplot +[mark=none, dotted, forget plot, color=red, thick] coordinates {(0.1, 0) (0.1, 1)};		
%		
%    	\addplot[
%   		color=orange,
%   		mark=diamond,
%   		mark repeat = 30,
%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/TROLL_noCCT};
%    	
%	\addplot[
%   		color=green!70!black,
%   		mark=x,
%   		mark repeat = 30,
%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/TROLL_Detach_noCCT};    	
%
%	\addplot[
%   		color=blue,
%   		mark=o,
%   		mark repeat = 30,
%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/TROLL_DetachPeriod};
%    	
%    	\addplot[
%   		color=black,
%%   		mark=triangle,
%%   		mark repeat = 30,
%%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/OLLA_0.03};
%    	
%    	\addplot[
%    		color=black,
%%    		mark=triangle,
%%   		    mark repeat = 30,
%		densely dashdotted,
%%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/OLLA_0.1};
%    	
%    	\addplot[
%    		color=black,
%%    		mark=triangle,
%%   		    mark repeat = 30,
%    		loosely dashed,
%%    	mark options={solid}
%    	]
%    	table[x expr=\thisrowno{0}*100, y index=1] {DataCDFs/Bler/OLLA_0.3};
%	\legend{\gls{TROLL}, \gls{TROLL} \gls{GD},  \gls{TROLL} \gls{GD}+ \gls{CCT}, OLLA 0.03, OLLA 0.1, OLLA 0.3}
